FactorJoin: A New Cardinality Estimation Framework for Join Queries

Cardinality estimation is one of the most fundamental and challenging problems in query optimization. Neither classical nor learning-based methods yield satisfactory performance when estimating the cardinality of the join queries. They either rely on simplified assumptions leading to ineffective cardinality estimates or build large models to understand the data distributions, leading to long planning times and a lack of generalizability across queries. In this paper, we propose a new framework FactorJoin for estimating join queries. FactorJoin combines the idea behind the classical join-histogram method to efficiently handle joins with the learning-based methods to accurately capture attribute correlation. Specifically, FactorJoin scans every table in a DB and builds single-table conditional distributions during an offline preparation phase. When a join query comes, FactorJoin translates it into a factor graph model over the learned distributions to effectively and efficiently estimate its cardinality. Unlike existing learning-based methods, FactorJoin does not need to de-normalize joins upfront or require executed query workloads to train the model. Since it only relies on single-table statistics, FactorJoin has small space overhead and is extremely easy to train and maintain. In our evaluation, FactorJoin can produce more effective estimates than the previous state-of-the-art learning-based methods, with 40x less estimation latency, 100x smaller model size, and 100x faster training speed at comparable or better accuracy. In addition, FactorJoin can estimate 10,000 sub-plan queries within one second to optimize the query plan, which is very close to the traditional cardinality estimators in commercial DBMS.

==> cover.tex <==
\section*{Revision summary}

We would like to thank all reviewers and meta-reviewers for their constructive suggestions for revision. We have addressed all question, concerns, and suggestions listed expect for a few minor issues.

Specifically, we 

==> experiments_old.tex <==
\section{Experiments and Evaluations}
\label{sec: experiments}

In this section, we empirically demonstrate the advantages of our framework over existing \CE methods. We first introduce the datasets, baselines to compare with, and experimental environment in Section~\ref{subsec: setups}. In the rest of this section, we would like to explore the following questions:

\noindent $\bullet$  \textbf{Overall performance} (Section~\ref{subsec: e2e}): how much improvement can our method achieve in terms of end-to-end query time? What are the model size and training time?

\noindent $\bullet$ \textbf{Detailed analysis} (Section~\ref{subsec: practicality}):
Why can our method attain good overall performance? When does our method perform better or worse than existing baselines?

\noindent $\bullet$ \textbf{Ablation study} (Section~\ref{subsec: ablation}):
How much does each optimization technique of this framework contribute to the overall performance?


\subsection{Experimental setups}
\label{subsec: setups}

\noindent\textbf{\underline{Datasets:}} We evaluate the performance of our \CE framework on two well-established benchmarks: \emph{STATS-CEB}~\cite{han2021cardinality} and \emph{IMDB-JOB}~\cite{leis2015good}, whose statistics are summarized in Table~\ref{tab: dataset}. We believe they represent the most comprehensive and challenging real-world benchmarks for \CE evaluation.

The \emph{STATS-CEB} benchmark uses the real-world dataset STATS, which is an anonymized dump of user-contributed content on
the Stack Exchange network. 
This dataset is consist of $8$ tables with overall $34$ columns and more than one million rows. 
It contains a large number of attribute correlations and distribution skewness, thus very challenging for the \CE.
The \emph{STATS-CEB} query workload contains $146$ queries involving $70$ different join templates with real-world semantics.
The true cardinalities of these queries range from $200$ to $2 \cdot 10^{10}$.
Some queries take more than one hour to execute in Postgres.
Worth noticing that \emph{STATS-CEB} benchmark only has star or chain join templates and numerical or categorical filtered attributes, thus friendly to evaluate all existing \CE baselines.

The \emph{IMDB-JOB} benchmark uses the real-world international movie database (IMDB). This dataset is comprised of $21$ tables with overall more than fifty million rows.
The \emph{IMDB-JOB} query workload contains $113$ queries with $33$ different join templates.
Some queries have more than $10,000$ sub-plan queries, posing a significant challenge to the efficiency of \CE methods.
Worth noticing that \emph{IMDB-JOB} benchmark contains cyclic joins and string pattern matching filter predicates. Therefore, the existing learned data-driven methods can not support this benchmark.


\smallskip
\noindent\textbf{\underline{Baselines:}} We compare our framework with the most competitive baselines in each \CE method category.

1) \emph{PostgreSQL}~\cite{psql2020} refers to the histogram-based \CE method
used in the well-known DBMS PostgreSQL. 

2) \emph{WJSample}~\cite{li2016wander} uses a random walk based-method called wander join to generate samples on the join of multiple tables. Its superior performance over the traditional sampling-based methods~\cite{bibid} has been demonstrated in recent studies~\cite{li2016wander, zhao2018random, park2020g}.

3) \emph{MSCN}~\cite{kipf2018learned} is a learned query-driven method based on multi-set
convolutional network model. 
On both datasets, we train MSCN on $100,000$ executed training queries that have roughly the same distribution as our testing query workloads.


4) \emph{BayesCard}~\cite{wu2020bayescard}, 5) \emph{DeepDB}~\cite{hilprecht2019deepdb}, and 6) \emph{FLAT}~\cite{zhu2020flat} are the SOTA learned data-driven \CE methods. They all use fanout methods to understand the data distributions of all join templates and estimate the join queries. Then, they apply different distribution models (Bayesian networks, sum-product networks~\cite{poon2011sum}, factorized sum-product networks~\cite{wu2020fspn}, respectively) to capture the data distribution on single tables or denormalized join tables.
We test these methods on \emph{STATS-CEB} only using the optimally-tuned model parameters~\cite{han2021cardinality}, because they can not support the \emph{IMDB-JOB}.

7) \emph{PessEst}~\cite{cai2019pessimistic} is the SOTA bound-based method, which leverages randomized hashing and data sketching to tighten the bound for multi-join queries. Its estimation has been verified to be very effective in real-world DBMS.
We use the best-tuned hyperparameters to evaluate PessEst on both benchmarks.

8) \emph{U-Block}~\cite{hertzschuch2021simplicity} uses top-k statistics to estimate the cardinality bound. The original paper designed a new plan enumeration strategy to work with this bound and showed promising results on \emph{IMDB-JOB}. However, for fair comparison, we only evaluate the standalone U-Block \CE method.

9) \emph{TrueCard} is the baseline that outputs the true cardinality of the query with no estimation latency. This baseline does not refer to any existing methods but it represents the optimal performance a \CE method can ever achieve.

We omit to compare with most of the other \CE methods~\cite{bruno2001stholes, srivastava2006isomer, khachatryan2015improving, fuchs2007compressed, stillger2001leo, wu2018towards, heimel2015self,kiefer2017estimating, leis2017cardinality, hasan2020, yang2020neurocard, wu2021uae, dutt2019selectivity} because the aforementioned baselines either have direct improvements or demonstrate clear advantages over these methods on various aspects~\cite{han2021cardinality}. In addition, some newly proposed methods~\cite{sun2019end, wang2021face, liu2021fauce} do not yet provide their open-source implementations for us to compare.

We implement our framework in Python mainly using numpy package. Regarding the hyperparameters of our framework, we assume no knowledge of the query workload and set the bin size $k$ to $100$ for both datasets. 
We use the BN-based \CE method~\cite{wu2020bayescard} as the single-table estimators for \emph{STATS-CEB} benchmark because this method is shown to be very accurate, fast, and robust for single table estimations.
For \emph{IMDB-JOB}, we use random sampling with $1\%$ sampling rate as the single-table estimators because this benchmark contains very complicated filter predicates such as disjunction and string pattern matching, which is not supported by the learned data-driven methods. 
We discuss and compare other hyperparameters of our framework in Section~\ref{subsec: ablation}.

\begin{table}[t]
	\scalebox{0.78}{
		\begin{tabular}{c|c|cc}
			\thickhline
			Category &Statistics &  STATS-CEB & IMDB-JOB \\ \thickhline
			\multirow{5}{*}{Data} & \# of tables & 8 & 21  \\ \cline{2-4}
			& \# of rows in each table & $10^3$ --- $4 \cdot 10^5$ & 6 --- $3 \cdot 10^7$ \\ \cline{2-4}
			& \# of columns in each table & 3 --- 10 & 2-12 \\ \cline{2-4}
			& \# of join keys & 13 & 36 \\ \cline{2-4}
			& \# of equivalent key groups & 2 & 11 \\ \thickhline
			\multirow{7}{*}{Query} & \# of queries & 146 & 113 \\ \cline{2-4}
			&\# of join templates & 70 & 33  \\ \cline{2-4}
			&join template type & star \& chain & +cyclic\\ \cline{2-4}
			&\# of filter predicates & 1 --- 16 & 1 --- 13  \\ \cline{2-4}
			&filter attributes & numerical \&  categorical & +string LIKE \\ \cline{2-4}
			&\# of sub-plan queries & 1 --- 75 & 8 --- $1 \cdot 10^4$ \\ \cline{2-4}
			&true cardinality range & 200 --- $2\cdot10^{10}$  & 1 --- $4 \cdot 10^6$  \\ \cline{2-4}
			&Postgres runtime (s) & 0.05 --- $10^{4}$  & $5 \cdot 10^{-4}$ --- 450 \\
			\thickhline
		\end{tabular}
	}
	\caption{Summary of STATS-CEB and IMDB-JOB benchmark.}
	\vspace{-2em}
	\label{tab: dataset}
\end{table}

\smallskip
\noindent\textbf{\underline{Environment:}}
We use the open-source implementation of all aforementioned baselines and best-tune their methods in both datasets to optimize their performance. 
All experiments are performed on a Ubuntu server with Intel Core Processor CPU having 20 cores, 57GB DDR4 main memory, and 300GB SSD.
For end-to-end evaluation, we integrate our framework along with all the baselines into the query optimizer of Postgres 13.1 following the procedure described in the recent benchmark work~\cite{han2021cardinality, han2021code}. 
Same as this prior work, we build all primary key and foreign key indexes and disable parallel computing in Postgres.
Specifically, we inject into Postgres all sub-plan query cardinalities estimated by each method, force the Postgres optimizer to use our injected cardinalities to optimize the query plan, and record the end-to-end query runtime (planning plus execution time). 
To eliminate the effect of memory cache, we first execute each workload multiple times. Then, we run the queries $3$ times for each method and record their average.




\subsection{Overall performance}
\label{subsec: e2e}

The most straightforward criterion to evaluate the performance of a \CE method is to test how much can a method improve the end-to-end query performance inside the query optimizer. Therefore, we compare and analyze the end-to-end performance along with the model size and training time of our framework and other baselines on \emph{STATS-CEB} and \emph{IMDB-JOB} benchmarks.

\begin{figure}
	\centering
	\includegraphics[width=8cm]{fig/overall_stats.pdf}
	\vspace{-1em}
	\caption{Overall performance on STATS-CEB.}
	\label{fig: overall-stats}
	\vspace{-1em}
\end{figure}

\begin{table}[t]
	\scalebox{0.8}{
		\begin{tabular}{c|ccc}
			\thickhline
			Method &  End-to-end time & Exec. + plan time & Improvement \\ \thickhline
			Postgres & 9.81h  &  9.81h + 25s & -- \\ \hline
			TrueCard  & 5.12h & 5.12h + 24s & 47.8\% \\ \hline
			WJSample & 16.52h & 16.51h + 45s & -68.4\% \\ \hline
			MSCN & 7.10h & 7.09h + 35s & 27.7\% \\ \hline
			BayesCard & 6.30h & 6.29h + 35s & 35.9\% \\ \hline
			DeepDB & 5.69h & 5.64h + 168s &  42.0\% \\ \hline
			FLAT & 5.36h & 5.24h + 437s & 45.3\% \\ \hline
			PessEst & 5.83h & 5.52h + 1135s & 40.5\% \\ \hline
			U-Block & 10.72h & 10.72h + 26s & -9.3\% \\ \hline
			\textbf{Ours} & \textbf{5.31h} & 5.30h + 36s & \textbf{45.8\%} \\ \thickhline
		\end{tabular}
	}
	\caption{End-to-end performance on STATS-CEB.}
	\vspace{-2em}
	\label{tab: STATS-CEB}
\end{table}


\smallskip
\noindent\textbf{\underline{Performance on STATS-CEB:}} 
We summarize the overall performance of all baselines in Figure~\ref{fig: overall-stats}.
We did not provide the model size and training time for \emph{Postgres}, \emph{TrueCard}, \emph{WJSample}, and \emph{U-Block} as they are negligible. 
In addition, we provide a detailed comparison of query execution and planning time (sum over all queries in the \emph{STATS-CEB}) in Table~\ref{tab: STATS-CEB}, with the relative improvement over \emph{Postgres} shown in the last column, i.e. (\emph{Postgres} - \emph{method}) / \emph{Postgres}.

Our framework achieves the best end-to-end query runtime ($5.31h$) among all baselines, which is close to optimal performance ($5.12h$ for \emph{TrueCard}). 
When compared with the traditional methods \emph{Postgres} and \emph{WJSample}, our framework has significantly better query execution time, indicating that our estimates are much more effective to generate high-quality query plans. 
Meanwhile, the planning time of our framework is close to \emph{Postgres}. 
This suggests that decomposing the join query into single-table \CE can lead to efficient estimates.

Judging from the pure query execution time in Table~\ref{tab: STATS-CEB}, our framework has comparable estimation effectiveness as the previous SOTA \emph{FLAT} on this benchmark. 
This learned data-driven method uses the fanout method to understand the distribution of all join patterns, which is accurate but very inefficient. Specifically, we can achieve better end-to-end performance than \emph{FLAT}, with $10$ times smaller planning time, $160$ times smaller model size, and $240$ times faster training time.
When compared to the other learned methods: \emph{BayesCard},  \emph{DeepDB}, and \emph{MSCN}, our framework can simultaneously achieve better query execution and planning time, smaller model size, and faster training time.
Therefore, we empirically verify that instead of modeling the distributions of all join patterns, accurately decomposing the join query into single-table estimates can generate equally effective but more efficient estimation with much smaller model size and training time.

Our framework and the SOTA bound-based method \emph{PessEst} can both generate very effective estimates. This observation verifies the claim that the bound-based method can produce effective estimates because it can help avoid very expensive query plans~\cite{cai2019pessimistic, atserias2008size, abo2017shannon, han2021cardinality}.
However, the planning time of \emph{PessEst} (1135s) is undesirable because it needs to materialize the tables after applying the filters and populate the upper bound during run-time.
Our framework has $35$ times less planning latency since instead of using exact bounds, we use probabilistic bounds derived from single-table estimates, which is  more efficient.


\begin{figure}
	\centering
	\includegraphics[width=6cm]{fig/overall.pdf}
	\vspace{-1em}
	\caption{Overall performance on IMDB-JOB (\revise{fake}).}
	\label{fig: overall-imdb}
	\vspace{-1em}
\end{figure}


\begin{table}[t]
	\scalebox{0.8}{
		\begin{tabular}{c|ccc}
			\thickhline
			Method &  End-to-end time & Exec. + plan time & Improvement \\ \thickhline
			Postgres & 2472s  &  2451s + 21s & -- \\ \hline
			TrueCard  & 375s & 358s + 17s & 84.8\% \\ \hline
			WJSample &  13618s & 12445s + 1173s & -450.9\% \\ \hline
			MSCN & 2024s  & 1937s + 87s  & 18.1\% \\ \hline
			PessEst & 4044s & 1230s + 2814s & -63.6\% \\ \hline
			U-Block & 2792s & 2762s + 30s & -12.9\% \\ \hline
			\textbf{Ours} & \textbf{1324s} & 1272s + 42s & \textbf{46.4\%} \\ \thickhline
		\end{tabular}
	}
	\caption{End-to-end performance on IMDB-JOB.}
	\vspace{-1em}
	\label{tab: IMDB-JOB}
\end{table}


\smallskip
\noindent\textbf{\underline{Performance on IMDB-JOB:}} 
We have put the overall performance in Figure~\ref{fig: overall-imdb} and the detailed end-to-end time comparison in Table~\ref{tab: IMDB-JOB} for the \emph{IMDB-JOB} workload.
Recall that the learned data-driven methods can not support this benchmark.

Our framework achieves the best end-to-end query runtime ($1324s$) among all baselines.
Similar observations can be derived as on the \emph{STATS-CEB} workload, when compared to the traditional methods \emph{Postgres} and \emph{WJSample}. 
Similar to STATS-CEB, \emph{PessEst} achieves the best performance in term pure execution time but has much larger overhead and planning latency.
Our framework has comparable performance as \emph{PessEst} in terms of pure execution time. However, our planning time is $50$ times shorter than \emph{PessEst}, making our framework much faster in overall end-to-end query time. Specifically, our framework can estimate $10,000$ sub-plan queries within one second, which is close to \emph{Postgres}.

However, unlike in \emph{STATS-CEB} where we have near-optimal performance, there still exists a large gap between our method (1324s) and the optimal \emph{TrueCard} (375s). There are two possible explanations. First, our probabilistic bound error can accumulate with the number of joins. Compared to the \emph{STATS-CEB}, the \emph{IMDB-JOB} contains more than twice the number of joins in the queries. Therefore, the relative performance of our framework drops severely when shifting from \emph{STATS-CEB} to \emph{IMDB-JOB}. 
Second, the base-table filters in \emph{IMDB-JOB} contain a large amount of highly-selective predicates, making our sampling-based single-table \CE less accurate. 
These observations suggest a room for improving our framework, which we discuss further in the future work section.

\smallskip
\noindent\textbf{\underline{Summary:}}
Our framework achieves the best performance among all the baselines on both benchmarks. 
Specifically, our framework can be as effective as the previous SOTA methods, and simultaneously be as efficient and practical as the tradition \CE methods. 
It is worth noting that, our framework is also very friendly for dynamic DBs with frequent data changes because we only need to update the single table \CE methods. This update procedure is clearly more efficient than existing learned methods, which either need to re-denormalize the join tables and re-calculate the fanout attributes~\cite{wu2020bayescard, hilp2019deepdb, zhu2020flat, yang2020neurocard} or need to gather new query workload to retrain the model~\cite{kipf2018learned, sun2019end}. 

%We leave the exploration of our model update as future work.\pari{again -- can move to future work section, or maybe even a stronger: It is clearly much easier to update these models, while past work in CE models such as NeuroCard,MSCN etc. (...), typically suggest to retrain the model as data is updated.}

\begin{figure}
	\centering
	\includegraphics[width=8.5cm]{fig/errors.pdf}
	\vspace{-2.5em}
	\caption{Relative estimation errors on \emph{STATS-CEB}.}
	\label{fig: errors}
	\vspace{-1em}
\end{figure}




\subsection{Detailed Analysis}
\label{subsec: practicality}
In this section, we first study why our framework can achieve the SOTA performance by analyzing the tightness of our probabilistic bound. 
Then, we exhaustively compare the \CE method's end-to-end performance on queries with different runtimes to investigate when can our framework perform better or worse than the competitive baselines. We only report the results of most representative methods (\emph{Postgres}, \emph{FLAT}, \emph{PessEst}) on \emph{STATS-CEB} and put the remaining results in the Appendix. 

\smallskip
\noindent\underline{\textbf{Bound tightness:}} 
We provide the relative error between our estimates and the true cardinalities (estimate / true) for all sub-plan queries on \emph{STATS-CEB} in Figure~\ref{fig: errors} with the following observations:

$\bullet$  Overall, all three SOTA methods significantly outperform \emph{Postgres} in terms of estimation accuracy. \emph{PessEst} generates exact upper bound and never underestimates. \emph{FLAT} understands the distributions of join patterns and produces the most accurate estimates.

$\bullet$  Our method can output an upper bound on cardinality for more than $90\%$ of the sub-plan queries. Most of the marginal underestimates have relative errors between $0.1$ and $1$, which can still generate relatively effective plans.

$\bullet$ The generated bounds of our method are slightly tighter than the bounds from \emph{PessEst}, which make our query plans more efficient to execute. 


\begin{figure}
	\centering
	\includegraphics[width=8.5cm]{fig/intervals.pdf}
	\vspace{-2.5em}
	\caption{Per query performance of \emph{STATS-CEB}.}
	\label{fig: intervals}
	\vspace{-1em}
\end{figure}

\smallskip
\noindent\underline{\textbf{Detailed comparision:}} We sort the $146$ queries of \emph{STATS-CEB} based on their Postgres end-to-end runtime and cluster them into $6$ different runtime intervals.
Figure~\ref{fig: intervals} reports relative improvements of the most competitive baselines over \emph{Postgres} for each query on the left and each cluster of queries on the right. 

For the very short-running queries (which could represent the OLTP workload), \emph{Postgres} is better among all methods, but our method can significantly outperform \emph{FLAT} and \emph{PessEst}. These methods perform worse because the estimation latency play a significant role in these queries.
We observe that improving estimation accuracy has a very limited effect on the query plan quality of short-running queries. This also explains why the optimal \emph{TrueCard} only marginally outperforms \emph{Postgres} on queries with less than $2s$ of runtime. 
%The estimation latency plays a significant role in these queries.
\emph{FLAT} and \emph{PessEst} are significantly worse than our method because their query latency significantly surpasses the execution time, which overshadows the minor improvement in query plans.

For the extremely long-running queries, the advantage of the SOTA methods over \emph{Postgres} gradually shows up. The reason is that estimation latency becomes increasingly insignificant for queries with a long execution time. Therefore, \emph{FLAT} and \emph{PessEst} which spend a long time planning can generate significantly better query plans. 


\subsection{Ablation study}
\label{subsec: ablation}

We conduct a series of ablation studies to analyze different optimization techniques in this framework. Specifically, we first investigate how do the number of bins (k) affect the overall performance. Then, we analyze the effectiveness of our new bin selection algorithm (GBSA introduced in Section~\ref{subsec: bin selection}) over the traditional equal-width and equal-depth bin selection algorithm. Finally, we study the performance of plugging-in different single-table \CE methods into our framework. Due to space limitations, we only provide the results on \emph{STATS-CEB}.\pari{skip the last line -- can just mention at the start of 6.2 that all the detailed analysis is only on stats-ceb, but imdb stuff is in the appendix, to avoid repeating this}

\smallskip
\noindent\underline{\textbf{Number of bins (k):}} 
We train our framework with five different values for the number of bins, ($1$, $10$, $50$, $100$, $200$), and evaluate them on \emph{STATS-CEB}.
Figure~\ref{fig: n_bins} shows the end-to-end query time (A), bound tightness (B), estimation latency per query (C), training time (D), and model size (E) of our framework.
For bound tightness, we report the $50\%, 95\%, 99\%$ percentiles of relative error: estimated/true, as the one used in Figure~\ref{fig: errors}.

Intuitively, the larger number of bins ($k$) will generate tighter cardinality bounds and thus more effective query plans, which is verified in Figure~\ref{fig: n_bins}-(A-B). 
Meanwhile, larger $k$ suggests large estimation latency, training time, and model size, which is verified in Figure~\ref{fig: n_bins}-(C-E). 
There are several interesting observations from these results.

$\bullet$ According to Figure~\ref{fig: n_bins}-(B), with $k=1$ (i.e. bin the entire domain of each join key into one bin) our framework can not generate tight bounds but it still outperforms \emph{Postgres} baseline by $24.9\%$. 
This highlights the importance of upper bounds over underestimation and verifies the effectiveness of bound-based algorithms.

$\bullet$ Increasing $k$ can drastically increase the bound tightness. However, at some point (from $k=100$ to $k=200$) the framework stopped producing better end-to-end performance. One explanation is that this fine-grained improvement in estimation accuracy can generate a slightly better query plan but the slower estimation latency cancels out the improvements in query plans. 

$\bullet$ The model size increases quadratically with $k$ because our framework has $O(N*k^2)$ complexity in both storage and inference. However, the estimation latency increases linearly with $k$ because the overall inference time is dominated by the single-table \CE inference time, whose complexity is linear with $k$. 


\begin{figure}
	\centering
	\includegraphics[width=8cm]{fig/ablation_bins.pdf}
	\vspace{-1.5em}
	\caption{Performance for different number of bins (x-axis).}
	\label{fig: n_bins}
	\vspace{-0.5em}
\end{figure}

\begin{table}[t]
	\scalebox{0.78}{
		\begin{tabular}{c|c|c|ccc}
			\thickhline
			\multirow{2}{*}{Algorithm} &  \multirow{2}{*}{End-to-end time} &  \multirow{2}{*}{Improvement} & \multicolumn{3}{c}{Bound Tightness (rel. error)} \\ \cline{4-6}
			& & & 50\% & 95\% & 99\% \\ \hline
			Equal-width & 6.63h & 32.4\%& 8.7 & 3135 & $2\times 10^5$ \\ \hline
			Equal-depth & 6.51h & 33.6\% & 8.4 & 2050 & $7 \times 10^4$ \\ \hline
			GBSA & 5.31h & 45.8\% &3.3 & 44 & 2782  \\ \thickhline
		\end{tabular}
	}
	\caption{Performance of different binning techniques.}
	\vspace{-1.5em}
	\label{tab: ablation-binning}
\end{table}

%\smallskip
\noindent\underline{\textbf{Different bin selection algorithms:}} Recall that in Section~\ref{subsec: bin selection}, we design a new algorithm, GBSA, to optimize the binning process for our framework. We compare it with the traditional equal-width and equal-depth binning algorithms. We set $k = 100$ for all three algorithms.
All algorithms have relatively the same estimation latency, training time, and model size. 
Thus, we only report the end-to-end performance and bound tightness in Figure~\ref{tab: ablation-binning}. 
We observe that GBSA can generate a much tighter upper bound, leading to significantly better end-to-end performance. This demonstrates the effectiveness of our GBSA algorithm.

%\smallskip
\noindent\underline{\textbf{Different plug-in single-table \CE methods:}} 
To compare the importance of single-table \CE methods in our framework, our framework plug-in three different types of estimators: 1) \emph{BayesCard} for a single table, which is the SOTA learned data-driven method, 2) \emph{Sampling}, which draws a random sample (5\%) from single tables on-the-fly and estimates the cardinalities of filter predicates, and 3) \emph{TrueScan} which scans and filters the tables during query time and calculate the true cardinality.

The end-to-end performance of different single table estimators with bin size $k=100$ is shown in Table~\ref{tab: single}. \emph{BayesCard} method performs significantly better than \emph{Sampling} because of more accurate estimates and slightly faster estimation speed. \emph{TrueSacn} produces an exact upper bound of the cardinalities and thus generates more effective query plans. However, the estimation latency is too high, making its overall end-to-end performance worse than \emph{BayesCard}.

\begin{table}[t]
	\scalebox{0.8}{
		\begin{tabular}{c|ccc}
			\thickhline
			Method &  End-to-end time & Exec. + plan time & Improvement \\ \hline
			BayesCard & 5.31h  &  5.30h + 36s & 45.8\% \\ \hline
			Sampling  & 5.73h & 5.72h + 41s & 41.6\% \\ \hline
			TrueScan & 5.37h & 5.21h + 578s & 45.3\% \\ \thickhline
		\end{tabular}
	}
	\caption{Performance of different single-table \CE.}
	\vspace{-2em}
	\label{tab: single}
\end{table}


\smallskip
\noindent\underline{\textbf{Summary:}} 
With a reasonable bin size $k$, our method can generate very tight bound with effective query plans. The GBSA bin selection algorithm is very effective in generating high-quality plans. Single-table \CE methods do have an impact on our framework's overall performance and we should choose one that can generate effective and efficient single-table estimates.
Overall, all different settings/hyperparameters of our framework can significantly outperform \emph{Postgres} baseline, verifying the robustness and stability of our framework.







